Streaming Radiance Fields for 3D Video Synthesis

We present an explicit-grid based method for efficiently reconstructing streaming radiance fields for novel view synthesis of real world dynamic scenes. Instead of training a single model that combines all the frames, we formulate the dynamic modeling problem with an incremental learning paradigm in which per-frame model difference is trained to complement the adaption of a base model on the current frame. By exploiting the simple yet effective tuning strategy with narrow bands, the proposed method realizes a feasible framework for handling video sequences on-the-fly with high training efficiency. The storage overhead induced by using explicit grid representations can be significantly reduced through the use of model difference based compression. We also introduce an efficient strategy to further accelerate model optimization for each frame. Experiments on challenging video sequences demonstrate that our approach is capable of achieving a training speed of 15 seconds per-frame with competitive rendering quality, which attains $1000 \times$ speedup over the state-of-the-art implicit methods. Code is available at https://github.com/AlgoHunt/StreamRF.

==> preliminaries.tex <==
\section{preliminaries}

\textcolor{cyan}{treat 3d video synthesis as training a sequence of 3d plenoptic scene representation} 

To rendering a static scene, Neural Radiance fields (NeRF)\cite{NeRF} learns a continuous mapping function between a 5D coordinate,(\ie 3D spatial position $\mathbf{x} \in \mathbb{R}^3$ with a view direction $\mathbf{d} \in \mathbb{R}^3$ , represented as a Cartesian unit vector)  to a corresponding volume density $\sigma \in \mathbb{R}$ and view-dependent color $\mathbf{c} \in \mathbb{R}^3$. The origin NeRF apply a multilayer perceptron (MLP) networks $f_{m}: (\mathbf{x}, \mathbf{d}) \mapsto (\mathbf{c}, \sigma)$ to approximate the mapping function. It then use a differentiable volume rendering to get the color $\hat{C}(\mathbf{r})$ of an given ray, by integrate sampled density and color along the ray: 

\begin{equation}\label{eq:render} 
    \widehat{C}(\mathbf{r}) = \sum_{i=1}^N T_i\cdot \alpha_i \cdot \mathbf{c}_i,
\end{equation}
\begin{equation}\label{eq:alpha_t}
    \alpha_i = 1 - \exp(-\sigma_i \delta_i),\quad T_i = \prod_{j=1}^{i-1} (1 - \alpha_j),
\end{equation}

Here $\alpha_i$ is the ray termination probability at the point $i$, $T_i$ represents how much light have transmitted when reaching at $i$, and $\delta_i$ is the adjacent points distance. In practice, photometric loss of a batch of rays between their predicted colors and the corresponding ground truths in the training images was used to train a typical NeRF network.

Based on the advantage and flexibility provided by this implicit formulation, N3DV smoothly extend NeRF to the dynamic scene by extending the 5D input into 6D input.But this also causes them to bear the corresponding disadvantages. suffer from the extremely costing training and rendering due  to every sample point need to passes through the mlp network. 

\answerTODO{} \textbf{modify this paragraph}

Recent advances, representative by Plenoxel \cite{yu2021plenoxels}, show that representing a scene as a discretized voxel grid and storing the corresponding properties in an explicit manner has significant advantages on training and inference efficiency, enabling real-time rendering. Formally, the volume density and the features inducing view-variant colors are respectively represented as $\mathbf{V}_{\sigma} \in \mathbb{R}^{H\times W\times K}$ and $\mathbf{V}_{c} \in \mathbb{R}^{H\times W\times K\times C}$. Here $H$, $W$ and $K$ correspond to the spacial resolutions of the grid. Particularly, the color information is described by employing a set of spherical harmonics (SH) in which the coefficients act as features (the dimension is $C$) to be optimized and can be inferred directly given the target viewing direction, allowing much higher efficiency on training and inference compared to the implicit representation methods.

\answerTODO{} \textbf{explain why we can not directly extend 3d grid to 4d grid as n3dv}



